A2RBench: An Automatic Paradigm for Formally Verifiable Abstract Reasoning Benchmark Generation

Abstract reasoning ability reflects the intelligence and generalization capacity of LLMs to extract and apply abstract rules. However, accurately measuring this ability remains challenging: existing benchmarks either rely on expensive manual annotation, limiting their scale, or risk measuring memorization rather than genuine reasoning. To address this, we introduce an automated pipeline named A2RBench, encompassing generation, expansion, evaluation, and analysis. Specifically, in the generation stage, LLMs create diverse tasks demanding genuine reasoning; in the expansion stage, LLMs reuse validated rules and expand new input spaces to generate task variations, achieving scaling. However, such a process may cause hallucinations. To eliminate it, we further establish a theoretical framework and prove that programmatic verification--testing whether the inverse operation perfectly reverses the forward operation (cycle consistency)--guarantees a unique solution. Through extensive evaluations on mainstream LLMs, we find: (1) Current LLMs exhibit fundamental deficiencies in abstract reasoning, with top models significantly underperforming humans on a representative subset (39.8% vs. 68.5%). (2) Current LLMs fall far short of 2D and 1D in the complexity of generated 3D tasks, revealing their lack of understanding of high-dimensional tasks. (3) Counterintuitively, inputs with higher information complexity can simplify the reasoning process.

==> content/resources/math_macro.tex <==
\newcommand{\seedmoe}{Seed-MoE}

==> content/resources/packages.tex <==
\usepackage{xargs}
\usepackage{todonotes}
\usepackage{tabularx}


==> template/mac_automl_core.tex <==
% =============================================================================
% MAC-AutoML core template
% Public responsibility:
% 1. Load all shared packages and layout rules.
% 2. Expose shared front-matter and header/footer configuration APIs.
% 3. Keep all theme-independent visual logic in one place.
%
% Theme wrappers are expected to define:
% - \macframecolordef
% - \macaccentcolordef
% - \macaccenttext
% =============================================================================

\@ifundefined{macframecolordef}{\ClassError{\@classname}{Missing theme hook \string\macframecolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccentcolordef}{\ClassError{\@classname}{Missing theme hook \string\macaccentcolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccenttext}{\ClassError{\@classname}{Missing theme hook \string\macaccenttext}{Define it in the theme .cls before loading mac_automl_core.tex}}{}

\newif\ifmacsubmissionmode
\newif\ifmacanonymousmode
\macsubmissionmodefalse
\macanonymousmodefalse

\DeclareOption{submission}{\macsubmissionmodetrue}
\DeclareOption{review}{\macsubmissionmodetrue}
\DeclareOption{cameraready}{\macsubmissionmodefalse}
\DeclareOption{camera-ready}{\macsubmissionmodefalse}
\DeclareOption{final}{\macsubmissionmodefalse}
\DeclareOption{anonymous}{\macanonymousmodetrue}
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions\relax

\LoadClass{article}
\RequirePackage{iftex}
\ifdefined\pdfoutput
\pdfoutput=1
\fi

% =============================================================================
% Core packages and layout
% =============================================================================

\RequirePackage[top=2.12cm, bottom=3.20cm, left=2.5cm, right=2.5cm, columnsep=0.65cm]{geometry}
\ifXeTeX\else
\RequirePackage{microtype}
\fi
\RequirePackage{placeins}
\RequirePackage{setspace}
\RequirePackage{parskip}
\RequirePackage[english]{babel}
\RequirePackage{lipsum}
\RequirePackage{etoolbox}
\RequirePackage{enumitem}
\newcommand{\nohyphens}{\hyphenpenalty=10000\exhyphenpenalty=10000\relax}

\RequirePackage{fancyhdr}
\@ifundefined{DisableLigatures}{}{\DisableLigatures[f]{family=sf*}}

% =============================================================================
% Graphics
% =============================================================================

\RequirePackage{graphicx}
\RequirePackage[export]{adjustbox}
\RequirePackage{subcaption}

% =============================================================================
% Tables
% =============================================================================

\RequirePackage{booktabs}
\RequirePackage{nicematrix}
\RequirePackage{multirow}
\RequirePackage{makecell}
\RequirePackage{colortbl}
\RequirePackage{bm}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\ifmacsubmissionmode
  \RequirePackage[switch,mathlines]{lineno}
  \AtBeginDocument{%
    \modulolinenumbers[1]%
    \linenumbers
  }
\fi
\RequirePackage{pifont}
\RequirePackage{marvosym}
\newcommand{\nm}[1]{#1}

% =============================================================================
% Theme colors
% =============================================================================

\RequirePackage[most]{tcolorbox}
\RequirePackage{xcolor}
\macframecolordef
\macaccentcolordef
\newcommand{\omniaccent}[1]{\macaccenttext{#1}}
\definecolor{black}{rgb}{0,0,0}
\newcommand{\black}[1]{{\bfseries\color[HTML]{000000} #1}}
\definecolor{macreviewnote}{RGB}{172,73,0}

% =============================================================================
% References
% =============================================================================

\RequirePackage{hyperref}
\RequirePackage{xurl}
\RequirePackage[noabbrev,nameinlink]{cleveref}
\hypersetup{
  colorlinks,
  linkcolor=omniaccent,
  citecolor=omniaccent,
  urlcolor=omniaccent
}

\RequirePackage[authoryear,round]{natbib}
\def\bibfont{\small}
\special{pdf:minorversion 7}
\emergencystretch=1.5em
\hbadness=2000

% =============================================================================
% Bibliography
% =============================================================================
\addto{\captionsenglish}{\renewcommand{\refname}{References}}
\newcommand{\citeas}[1]{\Needspace*{8\baselineskip}\noindent\bibentry{#1}}

% =============================================================================
% Section and caption style
% =============================================================================

\newcommand{\sectionfont}
{\fontsize{13}{14}\selectfont}

\newcommand{\subsectionfont}
{\fontsize{11}{13}\selectfont}

\RequirePackage{titlesec}
\titleformat*{\paragraph}{\itshape}
\titleformat*{\section}{\sectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsection}{\subsectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsubsection}{\normalsize\sffamily\bfseries\omniaccent}
\titlespacing*{\section}{0pt}{3ex plus4pt minus3pt}{5pt}
\titlespacing*{\subsection}{0pt}{2.5ex plus3pt minus2pt}{2pt}
\titlespacing*{\subsubsection}{0pt}{2ex plus2.5pt minus1.5pt}{2pt}

\RequirePackage{caption}
\DeclareCaptionLabelSeparator{period}{. }
\captionsetup{
  labelfont={bf,sf},
  labelsep=period,
  figurename=Figure,
  tablename=Table,
  format=plain,
  singlelinecheck=off,
  justification=raggedright,
  font=small
}
\captionsetup[figure]{
  skip=6pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}
\captionsetup[table]{
  skip=4pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}

\ifXeTeX
  \RequirePackage{fontspec}
  \IfFontExistsTF{TeX Gyre Termes}{%
    \setmainfont[
      SmallCapsFeatures = {Letters=SmallCaps}
    ]{TeX Gyre Termes}%
  }{%
    \IfFontExistsTF{Nimbus Roman}{%
      \setmainfont[
        SmallCapsFeatures = {Letters=SmallCaps}
      ]{Nimbus Roman}%
    }{%
      \setmainfont[
        SmallCapsFeatures = {Letters=SmallCaps}
      ]{Times New Roman}%
    }%
  }
  \IfFontExistsTF{Noto Sans}{\setsansfont{Noto Sans}}{\setsansfont{Arial}}
  \IfFontExistsTF{Noto Sans Mono}{\setmonofont{Noto Sans Mono}}{\setmonofont{Consolas}}
  \newfontfamily\omnibytesansmedium[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Medium,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Medium}
  \newfontfamily\omnititlefont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniheadingfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniauthorfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \IfFontExistsTF{Noto Sans}{%
    \newfontfamily\omniaffiliationfont[
      BoldFont = {Noto Sans SemiBold}
    ]{Noto Sans}
    \newfontfamily\omniemailfont[
      BoldFont = {Noto Sans SemiBold}
    ]{Noto Sans}
  }{%
    \newfontfamily\omniaffiliationfont[
      BoldFont = {Arial Bold}
    ]{Arial}
    \newfontfamily\omniemailfont[
      BoldFont = {Arial Bold}
    ]{Arial}
  }
  \IfFontExistsTF{Noto Sans Mono}{\newfontfamily\omnimonofont{Noto Sans Mono}}{\newfontfamily\omnimonofont{Consolas}}
\else
  \RequirePackage[T1]{fontenc}
  \renewcommand{\sfdefault}{lmss}%
  \renewcommand{\rmdefault}{cmr}
\fi

% =============================================================================
% Front-matter data model
% =============================================================================

\renewcommand\addtolist[5][]{
  \begingroup
    \if\relax#3\relax\def\sep{}\else\def\sep{#5}\fi
    \let\protect\@unexpandable@protect
    \xdef#3{\expandafter{#3}\sep #4[#1]{#2}}%
  \endgroup
}

\newcommand{\authorfont}
{\fontsize{12}{14}\selectfont}

\newcommand{\authorgroupfont}
{\fontsize{9.1}{10.8}\selectfont}
\newcommand{\affmark}[1]{\textsuperscript{#1}}

\newcommand\authorlist{}
\ifXeTeX
\newcommand\authorformat[2][]{\authorfont {\color{black!84}\omniauthorfont\bfseries #2\affmark{#1}}}
\else
\newcommand\authorformat[2][]{\authorfont {\color{black!82}\sffamily\mdseries #2\affmark{#1}}}
\fi
\renewcommand\author[2][]{\addtolist[#1]{#2}{\authorlist}{\authorformat}{, }}

\newcommand{\affiliationfont}
{\fontsize{10}{12}\selectfont}

\newcommand\affiliationlist{}
\ifXeTeX
\newcommand\affiliationformat[2][]{{\affiliationfont {\omniaffiliationfont \affmark{#1}#2}}}
\else
\newcommand\affiliationformat[2][]{{\affiliationfont {\sffamily \affmark{#1}#2}}}
\fi
\newcommand\affiliation[2][]{\addtolist[#1]{#2}{\affiliationlist}{\affiliationformat}{, }}

\newcommand{\contributionfont}
{\fontsize{9.6}{12}\selectfont}

\newcommand\contributionlist{}
\newcommand\contributionformat[2][]{{\contributionfont \affmark{#1}#2}}
\newcommand\contribution[2][]{\addtolist[#1]{#2}{\contributionlist}{\contributionformat}{, }}

\newcommand{\emailfont}
{\fontsize{8.2}{10.4}\selectfont}

\newcommand\emaillist{}
\ifXeTeX
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!60}\omniemailfont #1}}}
\else
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!65}\ttfamily #1}}}
\fi

\newcommand{\checkdatafont}
{\fontsize{7.92}{10}\selectfont}

\newcommand\checkdatalist{}
\newcommand\checkdataformat[2][]{{\small {\checkdatafont\sffamily \bfseries #1:} #2}}
\newcommand\checkdata[2][]{\addtolist[#1]{#2}{\checkdatalist}{\checkdataformat}{\par}}

\newcommand{\abstractinfont}
{\fontsize{10}{12}\selectfont}

\renewcommand{\abstract}[1]{\def\abstractlist{{\abstractinfont #1}}}
\newcommand{\email}[1]{\href{mailto:#1}{\texttt{#1}}}
\newcommand{\corremailmark}{\Letter}
\newcommand{\authormark}[1]{\textsuperscript{#1}}
\newcommand{\authorentry}[2]{\mbox{#1\authormark{#2}}}
\newcommand{\authorsep}{\hspace{0.78em}}
\newcommand{\authorrow}[1]{\makebox[\linewidth][c]{#1}\par\vspace{2.2pt}}
\newcommand{\affiliationline}[1]{#1\par}
\newcommand{\contactline}[1]{#1\par}

\newcommand{\macauthorrows}{}
\newcommand{\macaffiliationrows}{}
\newcommand{\maccontactrows}{}

% Public front-matter configuration API.
\newcommand{\setauthorrows}[1]{\gdef\macauthorrows{#1}}
\newcommand{\setaffiliationrows}[1]{\gdef\macaffiliationrows{#1}}
\newcommand{\setcontactrows}[1]{\gdef\maccontactrows{#1}}
\newcommand{\usecustomauthorlayout}{
  \def\authorlist{%
    {\fontsize{12}{14}\selectfont\color{black!96}%
    \ifXeTeX\omniauthorfont\bfseries\else\sffamily\bfseries\fi
    \parbox{0.96\linewidth}{\centering \macauthorrows}}}
  \def\affiliationlist{%
    {\fontsize{9.9}{11.9}\selectfont\color{black!70}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \parbox{0.92\linewidth}{\centering
    \macaffiliationrows\par
    \vspace{2.8mm}
    {\fontsize{9.8}{11.8}\selectfont\color{black!82}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \maccontactrows}}}}
  \def\emaillist{{}}}
\newcommand{\setfrontauthors}[1]{\setauthorrows{#1}}
\newcommand{\setfrontaffiliations}[1]{\setaffiliationrows{#1}}
\newcommand{\setfrontcontact}[1]{\setcontactrows{#1}}

\ifmacanonymousmode
  \AtBeginDocument{%
    \gdef\authorlist{%
      {\fontsize{12}{14}\selectfont\color{black!96}%
      \ifXeTeX\omniauthorfont\bfseries\else\sffamily\bfseries\fi
      Anonymous Authors}}%
    \gdef\affiliationlist{%
      {\fontsize{9.9}{11.9}\selectfont\color{black!70}%
      \ifXeTeX\omnibytesansmedium\else\sffamily\fi
      Affiliations withheld for double-blind review}}%
    \gdef\emaillist{}%
    \gdef\maccontactrows{}%
    \gdef\checkdatalist{}%
  }
\fi

\renewcommand\date[1]{\checkdata[Date]{#1}}
\newcommand\correspondence[1]{\checkdata[Correspondence]{#1}}

\newcommand{\titlefont}
{\fontsize{17}{20}\selectfont}

\ifXeTeX
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.945\linewidth}{\centering\titlefont{\omnititlefont\bfseries #1}}}}
\else
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.92\linewidth}{\centering\titlefont{\sffamily\bfseries #1}}}}
\fi

\newcommand{\abstractfont}
{\fontsize{12}{12}\selectfont}

\ifXeTeX
\newcommand{\beginabstract}{\abstractfont{\omniauthorfont\bfseries\color{omniaccent!88!black}Abstract}}
\else
\newcommand{\beginabstract}{\abstractfont{\sffamily\bfseries\color{omniaccent}\MakeUppercase{Abstract}}}
\fi

\newcommand{\beginappendix}{\appendix{\titlefont\sffamily \omniaccent{Appendix}\par}}
\colorlet{abstractboxfill}{white}

% =============================================================================
% Reusable document-level utilities
% =============================================================================

\newcommand{\macparagraph}[1]{\par\vspace{2pt}\noindent\textbf{#1}\hspace{1.8ex}}
\newcommand{\reviewnote}[1]{%
  \ifmacsubmissionmode
    {\color{macreviewnote}\bfseries [Review note: }{\color{macreviewnote}#1}{\color{macreviewnote}\bfseries ]}%
  \fi
}
\definecolor{macgreen}{RGB}{34,139,34}
\definecolor{macred}{RGB}{220,20,60}
\definecolor{macorange}{RGB}{255,140,0}
\newcommand{\cmark}{\textcolor{macgreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{macred}{\ding{55}}}
\newcommand{\pmark}{\textcolor{macorange}{\raisebox{0.12ex}{\footnotesize\textasciitilde}}}
\newcommand{\fb}{\makebox[0.5em][c]{\textbullet}}
\newcommand{\eb}{\makebox[0.5em][c]{\textopenbullet}}
\newcommand{\eg}{e.g.,\ }
\newcommand{\ie}{i.e.,\ }

\tcbuselibrary{skins}
\tcbset{
  aibox/.style={
    width=\linewidth,
    top=7pt,
    bottom=2pt,
    colback=blue!4!white,
    colframe=black,
    colbacktitle=black,
    enhanced,
    center,
    attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    boxed title style={boxrule=0pt,colframe=white,},
  }
}
\newtcolorbox{AIbox}[2][]{aibox,title=#2,#1}

% =============================================================================
% Template-level branding configuration
% =============================================================================

\newcommand{\macleftheadercontent}{}
\newcommand{\macrightheadericon}{}
\newcommand{\macrunningheadericon}{}
\newcommand{\macheadertextcontent}{MAC-AutoML}
\newcommand{\macreviewheaderlabel}{Submission / Review Copy}

\newcommand{\setleftheadercontent}[1]{\gdef\macleftheadercontent{#1}}
\newcommand{\setrightheadericon}[1]{\gdef\macrightheadericon{#1}}
\newcommand{\setrunningheadericon}[1]{\gdef\macrunningheadericon{#1}}
\newcommand{\setheadergroupname}[1]{\gdef\macheadertextcontent{#1}}
\newcommand{\setreviewheaderlabel}[1]{\gdef\macreviewheaderlabel{#1}}
\newcommand{\headerlogo}[3][0pt]{\raisebox{#1}{\includegraphics[height=#2]{#3}}}
\newcommand{\headerlogospace}[1]{\hspace*{#1}}

% Public header/footer configuration API.
\newcommand{\firstpageheaderlogos}{%
  \makebox[\textwidth][s]{%
    \macleftheadercontent\hfill\macrightheadericon
  }%
}
\ifXeTeX
\newcommand{\omniheadertext}{{\omniauthorfont\fontsize{8.1}{10}\selectfont\color{black!58}\addfontfeatures{LetterSpace=4}\macheadertextcontent\ifmacsubmissionmode\space/\space\macreviewheaderlabel\fi}}
\else
\newcommand{\omniheadertext}{\sffamily\fontsize{8.1}{10}\selectfont\color{black!60} \macheadertextcontent\ifmacsubmissionmode\space/\space\macreviewheaderlabel\fi}
\fi
\fancypagestyle{firststyle}{
    \fancyhead[L]{
        \vskip 0.8mm
        \firstpageheaderlogos
    }
    \fancyhead[R]{}
}
\pagestyle{fancy}
\fancyhf{}
\fancyhead[L]{
  \vskip 2.5mm
  \macrunningheadericon
}
\fancyhead[R]{
  \vskip 4.2mm
  \omniheadertext
}
\fancyfoot[C]{\sffamily\fontsize{8.6}{10}\selectfont\thepage}

\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}
\setlength{\headheight}{64pt}
\setlength{\headsep}{6pt}
\setlength{\footskip}{18pt}

% =============================================================================
% Title and abstract box implementation
% =============================================================================
\newcommand{\@toptitlebar}{
  {\color{omniaccent!88!black}\hrule height 2.4pt}
  \vskip 6mm
}
\newcommand{\@bottomtitlebar}{
  \vskip 6mm
  {\color{omniaccent!88!black}\hrule height 2.4pt}
}

% Titlebox %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mymaketitle}{%
  \tcbset{enhanced}
  \tcbset{left=8mm}
  \tcbset{right=8mm}
  \tcbset{top=4.0mm}
  \tcbset{bottom=3.8mm}
  \tcbset{colback=white}
  \tcbset{colframe=omniframe}
  \tcbset{boxrule=3pt}
  \tcbset{before skip=0pt}
  \tcbset{grow to left by=1.5pt}
  \tcbset{grow to right by=1.5pt}
  \tcbset{arc=2.2mm}
      {
      \setlength{\parskip}{0mm}
      \hfuzz=20pt
      \hbadness=10000
      \centering
      \nohyphens

      {
      \vspace*{-4.8mm}
      \@toptitlebar

        \ifmacsubmissionmode
          {\sffamily\fontsize{9.2}{11}\selectfont\bfseries\color{omniaccent!72!black}\macreviewheaderlabel\par}
          \vskip 2.4mm
        \fi
        \titlelist\par
         \@bottomtitlebar
      }
      \vskip 4.0mm
      \authorlist
      \vskip 2.4mm

      \affiliationlist\par
      \ifdefempty{\emaillist}{}{\vskip 3mm \emaillist\par}

      \contributionlist\par
    }
   \vskip 2.6mm

  \begin{tcolorbox}[
    enhanced jigsaw,
    colback=abstractboxfill,
    colframe=omniaccent!99,
    boxrule=1.6pt,
    arc=2.5mm,
    left=8mm,
    right=8mm,
    top=4.1mm,
    bottom=4.2mm,
    interior style={fill=abstractboxfill},
    drop shadow={black!12!white},
    before skip=0pt,
    after skip=0pt
  ]
    \setlength{\parindent}{0cm}
    \setlength{\parskip}{0cm}

    \begin{center}
      \beginabstract
      \vskip 1.8mm
    \end{center}

    \abstractlist\par
    \vskip 0.6mm
    {
      \setlength{\parskip}{0cm}
      \ifdefempty{\checkdatalist}{\vspace*{0.02cm}}{\checkdatalist\par}
      \ifmacsubmissionmode
        {\small {\checkdatafont\sffamily \bfseries Mode:} \macreviewheaderlabel\par}
      \fi
    }
  \end{tcolorbox}
  \tcbset{reset}
  \FloatBarrier

  \thispagestyle{firststyle}
}

\if@twocolumn%
\renewcommand{\maketitle}{
\twocolumn[%
 \vskip 2mm
  \mymaketitle
  \vskip 4mm
]
}%
\else%
\renewcommand{\maketitle}{
  \mymaketitle
  \vskip 4mm
}%
\fi


